Evolving Clustered Random Networks

We propose a Markov chain simulation method to generate simple connected random graphs with a specified degree sequence and level of clustering. The networks generated by our algorithm are random in all other respects and can thus serve as generic models for studying the impacts of degree distributions and clustering on dynamical processes as well as null models for detecting other structural properties in empirical networks.

==> bibliography.tex <==
\begin{thebibliography}{9}
\small  % Use 9 point text.
\bibitem{volz_clust}
Volz, E. (2004) Random networks with tunable degree distribution and
clustering. {\em Phys. Rev. E} 70, 056115

\bibitem{serrano}
Serrano, M., Boguna, M. (2006) Clustering in Complex Networks I.

\bibitem{boguna}
Serrano, M., Boguna, M. (2005) Tuning clustering in random networks
with arbitrary degree distributions. {\em Phys. Rev. E} 72, 036133

\bibitem{soffer}
Soffer, S., Vazquez, A. (2005) Network clustering coefficient
without degree-correlation biases. {\em Phys. Rev. E} 71, 057101

\bibitem{gkantsidis}
C. Gkantsidis, M. Mihail, and E. Zegura. The markov chain simulation
method for generating connected power law random graphs. In Proc.
5th Workshop on Algorithm Engineering and Experiments (ALENEX).SIAM,
January 2003

\bibitem{barab}
Albert, R., Barabasi, A.L. (2000) Topology of evolving networks.
{\em Phys Rev Lett.} 85(24):5234-7

\bibitem{ravasz}
Ravasz, E. and Barabasi, A.L. (2003) Hierarchical organization in
complex networks. Phys Rev E. 67, 026112.

\bibitem{mejn_clust}
Newman, M.E.J. Properties of highly clustered networks. Phys. Rev. E
68, 026121 (2003)

\bibitem{park}
Newman, M.E.J. and Juyong Park. Why social networks are different
from other types of networks. Phys. Rev. E 68, 036122 (2003)

\bibitem{trapman}
Trapman, P. On stochastic models for the spread of infections.

\bibitem{guil}
Guillaume, J. and Latapy, M. (2005) Bipartite Graphs as Models of
Complex Networks. Lecture Notes in Computer Science. Vol 3405,
127-139.

\bibitem{milo}
Milo, R., Kashtan, N., Itzkovitz, S., Newman, M.E.J, Alon, U. On the
uniform generation of random graphs with prescribed degree
sequences.

\bibitem{havel}
Havel, V. A remark on the existence of finite graphs. \emph{Caposis
Pest. Mat.}, 80:496-506, 1955

\bibitem{hakimi}
Hakimi, S.L. On the realizability of a set of integers as degrees of
the vertices of a liinear graph. \emph{SIAM Journal}. 10(3):496-506.
1962

\bibitem{erdos}
Erdos and Gallai. Graphs with prescribed degree of vertices.
\emph{Mat. Lapok.}, 11:264-274, 1960

\bibitem{taylor}
Taylor, R. Constrained switchings in graphs. \emph{Comb. Mat.}, 8,
1980.

\bibitem{maslov}
Maslov and Sneppen. Science 296, 910 (2002) ??

\bibitem{callaway}
Callaway, D.S.,J.E.Hopcroft,J.M.Kleinberg,M.E.J. Newman,S.H.Strogatz
Are randomly grown graphs really random? Phys. Rev. E 64, 041902
(2001).

\bibitem{netsci}M. E. J. Newman, Finding community structure in networks using the eigenvectors of matrices. Phys. Rev. E 74, 036104 (2006).

\bibitem{newman_watts} Newman, M.E.J., Watts, D.J., Strogatz, S.H.
Random graph models of social networks. Proc. Natl. Acad. Sci. 99,
2566 (2002).

\bibitem{keeling_invasion} Keeling, M.J. The effects of local spatial structure on epidemiological invasions.
Proc. R. Soc. B 266, 859-867 (1999).

\bibitem{watts} Watts, D., Strogatz, S.H., Collective Dynamics of Small World Networks, Nature 393, 441 (1998).

\bibitem{meyers_sars} Meyers, L.A., Pourbohloul, B., Newman, M.E.J., Skowronski, D.M., Brunham, R.C.
Network theory and SARS: predicting outbreak diversity. J. Theor.
Biol. 232, 71-81. (2005).

\bibitem{molloy_reed}Molloy, M., Reed, B. 1995 A critical point for random graphs with a given degree sequence. Random Struct. Algo.6:161

\bibitem{mejn_cs} Newman, M.E.J.  Detecting community structure in networks. \emph{Eur. Phys. J. B} \textbf{38}, 321-330 (2004).

\bibitem{albert_stat}Albert, R., Barabasi, A. L. 2002 Statistical mechanics of complex networks. Reviews of Modern Physics 74, 47-97.

\bibitem{albert_error}Albert, R., Jeong, H., Barabasi, A. L. 2000 Error and attack tolerance of complex networks. Nature 406, 378-382.

\bibitem{faloutsos}Faloutsos, M., Faloutsos, P., Faloutsos, C. 1999 On Power-Law Relationships of the Internet Topology.  Proceedings of the Conference on applications, technologies, architectures, and protocols for computer communications.

\bibitem{keeling_networks}Keeling, M.J., Eames, K.T.D. 2005 Networks and epidemic models. J. R. Soc. Interface. 2, 295-307

\bibitem{petermann}Petermann, T., Rios, P.D.L. 2004 The role of clustering and gridlike odering in epidemic spreading.  Phys Rev E. 69, 066116

\bibitem{albert}Albert, R., Jeong, H., Barabasi, A.-L. 1999 The diameter of the World Wide Web. Nature 401, 130-131.

\bibitem{pajek}
All graphs were produced using Pajek.

\bibitem{radicchi}
F. Radicchi, C. Castellano, F. Cecconi, V. Loreto, and D. Parisi.
Defining and identifying communities in networks. PNAS, 101(9), 2004

\bibitem{milo2}
R. Milo, S. Shen-Orr, S. Itzkovitz, N. Kashtan, D. Chklovskii and U.
Alon, Network Motifs: Simple Building Blocks of Complex Networks
Science, 298:824-827

\bibitem{vazquez2}
Vazquez A, Dobrin R, Sergi D, Eckmann JP, Oltvai ZN, Barabasi AL:
The topological relationship between the large-scale attributes and
local interaction patterns of complex networks. Proc Natl Acad Sci
USA 2004, 101:17940-51794

\bibitem{newman_cs} Newman, M.E.J.  Detecting community structure in networks. \emph{Eur. Phys. J. B} \textbf{38}, 321-330 (2004).

\bibitem{yeast}Characterization and modeling of protein-protein interaction networks
V. Colizza, A. Flammini, A. Maritan, A. Vespignani Physica A 352,
1-27 (2005)

\bibitem{airline_data}Bureau of Transportation Statistics, US
Department of Transporation: http://www.transtats.bts.gov/

\bibitem{www_graph}Pages linking to www.epa.gov from http://www.cs.cornell.edu/courses/cs685/2002fa/

\bibitem{mejn_ass}Newman, M.E.J. Assortative mixing in networks. Phys. Rev. Lett. 89, 208701 (2002).


\end{thebibliography}

